The Art of the Steal: Purloining Deep Learning Models Developed for an Ultrasound Scanner to a Competitor Machine

A transfer function approach has recently proven effective for calibrating deep learning (DL) algorithms in quantitative ultrasound (QUS), addressing data shifts at both the acquisition and machine levels. Expanding on this approach, we develop a strategy to 'steal' the functionality of a DL model from one ultrasound machine and implement it on another, in the context of QUS. This demonstrates the ease with which the functionality of a DL model can be transferred between machines, highlighting the security risks associated with deploying such models in a commercial scanner for clinical use. The proposed method is a black-box unsupervised domain adaptation technique that integrates the transfer function approach with an iterative schema. It does not utilize any information related to model internals of the victim machine but it solely relies on the availability of input-output interface. Additionally, we assume the availability of unlabelled data from the testing machine, i.e., the perpetrator machine. This scenario could become commonplace as companies begin deploying their DL functionalities for clinical use. Competing companies might acquire the victim machine and, through the input-output interface, replicate the functionality onto their own machines. In the experiments, we used a SonixOne and a Verasonics machine. The victim model was trained on SonixOne data, and its functionality was then transferred to the Verasonics machine. The proposed method successfully transferred the functionality to the Verasonics machine, achieving a remarkable 98\% classification accuracy in a binary decision task. This study underscores the need to establish security measures prior to deploying DL models in clinical settings.

==> theory.tex <==
\section{Theory}
\label{sec:theory}

\begin{comment}
    
Any form of learning algorithm would be ineffective if there are data mismatches between training and testing data, and no assumptions can be made to calibrate the mismatches. Ideally, we need to collect a large and diverse training data set at each imaging setting to completely eliminate data mismatches caused by scanner parameters. However, acquiring such a training data set can be extremely expensive. Another approach could be training on a subset of imaging settings, which makes the data generation and gathering process less expensive. However, there will still be generalization issues for the settings that are not included in the training set. The question we address here is "How can we mitigate acquisition-related data mismatches in an inexpensive and generalizable way for QUS?"

To accomplish this, we consider a systems response approach. Biomedical ultrasound imaging can be viewed as a system, which encodes all the information related to an imaging system working on a tissue signal, which encodes all the information related to an imaging substrate. Subsequently, an image obtained by an ultrasound imaging system can be decomposed into two parts: a system response and a tissue signal. Then, the problem of acquisition-related data mismatch can be posed as matching system responses. When training inputs and testing inputs are from different distributions due to different scanner settings, such as a different excitation pulse frequency, there are two different system responses in the imaging process, one corresponding to training and the other one corresponding to deployment or testing. Potentially, a function can be defined that allows a system to transfer from one environment to the other environment. 

More precisely, under a single scattering approximation and when at least one aperture diameter away from the transducer surface, the backscattered frequency spectrum from a medium can be represented as \cite{mamou2013quantitative}
\begin{align}
\label{powerspec_initial}
    W(f,\textbf{x}) = T(f,\textbf{x}) A(f,\textbf{x}) D(f,\textbf{x}) H(f) R(f,\textbf{x})
\end{align}
where $f$ represents frequency, $x$ represents axial direction, $T (f,\textbf{x})$ incorporates the transmission losses between tissues, $A(f,\textbf{x})$ is the frequency-dependent attenuation, $D(f,\textbf{x})$ represents the diffraction effects of the transducer, $H (f)$ is the impulse response of the transducer system and incorporates the electro-mechanical response, and $R(f,\textbf{x})$ is the scattering function describing the underlying tissue micro-structure. Therefore, an ultrasound image can be naively decomposed as 
\begin{align}
\label{powerspec_simple}
    W(f,\textbf{x}) = S_\phi(f,\textbf{x}) P(f,\textbf{x})
\end{align}
where $S_\phi(f,\textbf{x}) = D(f,\textbf{x}) H(f,\textbf{x}) $ is the system response which incorporates all the information related to ultrasound imaging system and $P(f,\textbf{x}) = T(f,\textbf{x}) A(f,\textbf{x})R(f,\textbf{x})$, which is the tissue or sample signal that incorporates all the information related to imaging substrate (i.e., attenuation, transmission losses and scattering function). The subscript $\phi$ in $S_\phi(f,\textbf{x})$ represents the scanner setting, exclusively $\phi_{train}$ stands for training environment and $\phi_{test}$ stands for testing environment, for later use. To calibrate the acquisition-related data mismatches between two system settings, we setup the scenario where the tissue signal, $P(f,\textbf{x})$, does not change between testing and training, such that,
\begin{align}
\label{powerspec}
   \frac{W_{test}(f,\textbf{x})}{W_{train}(f,\textbf{x})} &= \frac{S_{\phi_{test}}(f,\textbf{x})}{S_{\phi_{train}}(f,\textbf{x})}\\ &= \Gamma(f,\textbf{x})
\end{align}
where $\Gamma(f,\textbf{x})$ represents the\textit{ "setting transfer function" }between training and testing system parameters. This can be done in a practical way by selecting a tissue mimicking phantom with uniform scattering properties and fixing the transducer to scan and record the signal from a single location in the phantom while the settings are changed from training to testing. To calibrate in training time,  $\Gamma(f,\textbf{x})$ is sufficient:
\begin{align}
\label{training time}
    W_{test}(f,\textbf{x}) &= \Gamma(f,\textbf{x}) W_{train}(f,\textbf{x})
\end{align}
and hence, it is a convolution operation in time direction, $t$ 
\begin{align}
\label{training time_spatial_domain}
    w_{test}(t,\textbf{x}) &= \gamma_{train}(t,\textbf{x}) \ast_{t} w_{train}(t,\textbf{x})
\end{align}
where $\gamma_{train}$ represents the \textit{"setting transfer filter"} for training time. For the train-time calibration, a DL model is trained at testing data settings, and therefore, testing data can be input into the DL model directly. In order to achieve this, the training data are converted to the testing data via the setting transfer function $\Gamma(f,\textbf{x})$ in training time and a new model is developed by the network, which allows the testing data settings to match with training settings used to create the model. 

Similarly, $\Gamma^{-1}(f,\textbf{x})$ is sufficient for calibrating in testing time:
\begin{align}
\label{test time}
   W_{train}(f,\textbf{x}) &= \Gamma^{-1}(f,\textbf{x}) W_{test}(f,\textbf{x}),
\end{align}
which results in the following filtering operation
\begin{align}
\label{test time_spatial_domain}
    w_{train}(t,\textbf{x}) &= \gamma_{test}(t,\textbf{x}) \ast_{t} w_{test}(t,\textbf{x})
\end{align}
where $\gamma_{test}$ represents the \textit{"setting transfer filter"} for testing time. For the test-time calibration, a DL model is trained at the training data settings, and therefore, testing data can't be input into the DL model directly. The testing data needs to be converted to training data via the setting transfer function $\Gamma^{-1}(f,\textbf{x})$. Then, the model developed with the original training data and its associated settings are used with the converted testing data.  

In this work, we propose to use a signals and systems perspective to \textit{calibrate} training or testing data. Here is the proposed method step by step at a high-level:

\begin{itemize}
    \item[1.] Gather a \textit{large} amount of training data at a single setting.
    \item[2.] Gather a \textit{small} amount of calibration data at each scanner setting.
    \item[3.] Calculate $W_{test}$ or $W_{train}$ by using the calibration set to calculate the setting transfer function $\Gamma$ and $\Gamma^{-1}$
    \item[4.] Construct linear phase filters $\gamma_{train}$ or  $\gamma_{test}$ by using the magnitude responses of $\Gamma$ and $\Gamma^{-1}$.
    \item[5.] When a different setting than training setting is being used in the scanning process, calibrate the mismatch by using filters $\gamma_{train}$ or $\gamma_{test}$ either in the training time or in the testing time in the DL network, respectively.  
\end{itemize}

\end{comment}

